Consistent Client Simulation for Motivational Interviewing-based Counseling

Simulating human clients in mental health counseling is crucial for training and evaluating counselors (both human or simulated) in a scalable manner. Nevertheless, past research on client simulation did not focus on complex conversation tasks such as mental health counseling. In these tasks, the challenge is to ensure that the client's actions (i.e., interactions with the counselor) are consistent with with its stipulated profiles and negative behavior settings. In this paper, we propose a novel framework that supports consistent client simulation for mental health counseling. Our framework tracks the mental state of a simulated client, controls its state transitions, and generates for each state behaviors consistent with the client's motivation, beliefs, preferred plan to change, and receptivity. By varying the client profile and receptivity, we demonstrate that consistent simulated clients for different counseling scenarios can be effectively created. Both our automatic and expert evaluations on the generated counseling sessions also show that our client simulation method achieves higher consistency than previous methods.

==> sections/human_annotation.tex <==
\section{Expert Annotation}
\label{app:human evaluation}


\subsection{Demographics for Annotators}

Our annotation team comprises four experts who are co-authors of this paper. Three of them hold postgraduate degrees in counseling and one is a senior-year university student pursuing a psychology major. They all have relevant experience in mental health counseling.

\subsection{Annotation Instruction}

Table~\ref{tab:human_instruction1} presents the profile consistency rating score descriptions and client profile components for an expert to evaluate the profile consistency scores of a generated counseling session in all the four profile aspects (i.e., persona, beliefs, motivation, and acceptable plan). Table~\ref{tab:human_instruction2} shows the realism rating score descriptions for an expert to assess the realism of client in a generated session. Finally, Table~\ref{tab:human_instruction3} shows the score descriptions for an expert to determine the receptivity level of client in a generated counseling session.

\begin{table*}[tb]
\begin{tabularx}{\textwidth}{X}
\toprule
\textbf{Consistency Rating (To rate how consistent is the client with the four aspects of profile)}\newline
5 (High): Perfectly aligns with profile across all aspects \newline
4 (Moderately High): Mostly aligns with profile with minor variations \newline
3 (Moderate): Partially aligns with profile with some discrepancies \newline
2 (Moderately Low): Limited alignment with profile with multiple discrepancies \newline
1 (Low): Consistently contradicts profile information \newline
\textbf{CLIENT PROFILE} \newline
\textbf{Behavior:} drinking alcohol \newline
\textbf{Personas:}\newline
- The client sneaked out with a friend to the park to has a couple of beers.\newline
- The client managed to avoid getting into trouble as he threw the beers away before the policy saw them.\newline
- If the the client's mother found out he was in trouble because of his drinking, she would kill him.\newline
- The client has an interest in soccer and has set a goal to play in college.\newline
- The client has aspirations of receiving scholarships to support his soccer career.\newline
\textbf{Beliefs:} \newline
- The client believes he can handle the dangerous situation to avoid getting into trouble. \newline
- The client has only drunk once or twice. \newline
- A couple of the client's friends drink too. \newline
\textbf{Motivation:} The client is motivated because of the risk of drinking alcohol in sports, as alcohol would affect the ability to play soccer. \newline
\textbf{Acceptable Plans:} None \newline
\textbf{SESSION} \newline
[conversation]
\\ \bottomrule
\end{tabularx}
\caption{Description of profile consistency rating scores, ground truth client profile, and counseling session for expert annotation.  The expert is required to give a rating for each profile aspect. ([conversation] will be replaced by the real or generated session.)}
\label{tab:human_instruction1}
\end{table*}


\begin{table*}[tb]
\begin{tabularx}{\textwidth}{X}
\toprule
\textbf{Realism Rating (To rate how realistic is the client compared to a human client)} \newline
5 (High): Shows authentic responses with natural flow and rich personal context\newline
4 (Moderately High): Shows mostly genuine responses with occasional scripted moments\newline
3 (Moderate): Shows mixed authentic and artificial responses\newline
2 (Moderately Low): Shows mostly artificial responses with few authentic moments\newline
1 (Low): Shows completely artificial responses with no authentic elements\newline
\textbf{SESSION}\newline
[conversation]
\\ \bottomrule
\end{tabularx}
\caption{Description of realism rating scores, and counseling session for expert annotation. ([conversation] will be replaced by the real or generated session.)}
\label{tab:human_instruction2}
\end{table*}

\begin{table*}[tb]
\begin{tabularx}{\textwidth}{X}
\toprule
\textbf{Receptivity Rating (To rate how receptive is the client in the session)} \newline
5 (High): Actively engages, shares openly, and responds positively \newline
3 (Moderate): Shows balanced sharing and mixed response patterns \newline
1 (Low): Consistently withholds and strongly resists engagement \newline
\textbf{SESSION} \newline
[conversation]
\\ \bottomrule
\end{tabularx}
\caption{Description of receptivity ratings, and counseling session for expert annotation. ([conversation] will be replaced by the real or generated session.)}
\label{tab:human_instruction3}
\end{table*}


